An immersed boundary method for particle-resolved simulations of arbitrary-shaped rigid particles

The present work extends the direct-forcing immersed boundary method introduced by Garc\'ia-Villalba et al. (2023), broadening its application from spherical to arbitrarily-shaped particles, while maintaining its capacity to address both neutrally-buoyant and light objects (down to a density ratio of 0.5). The proposed method offers a significant advantage over existing methods regarding its simplicity, in particular for the case of neutrally-buoyant particles. Three test cases from the literature are selected for validation: a neutrally-buoyant prolate spheroid in a shear flow; a settling oblate spheroid; and, finally, a rising oblate spheroid.

==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MACROS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% GLOSSAR
\newcommand{\Deq}[1]{$D$}
\newcommand{\ddt}[1]{\frac{\text{d}#1}{\text{d} t}}
\newcommand{\ppt}[1]{\frac{\partial#1}{\partial t}}
\newcommand{\wrt}[1]{\text{d}#1}

%%% COLORS
\definecolor{color1}{HTML}{1B9E77} % dark teal
\definecolor{color2}{HTML}{D95F02} % dark orange
\definecolor{color3}{HTML}{7570B3} % dark lilac
\definecolor{color4}{HTML}{E7298A} % dark magenta
\definecolor{color5}{HTML}{66A61E} % dark lime green
\definecolor{color6}{HTML}{E6AB02} % dark banana
\definecolor{color7}{HTML}{A6761D} % dark tan
\definecolor{color8}{HTML}{666666} % dark gray
%-- TU master thesis
\definecolor{color_green}{HTML}{A9AE19} % green
\definecolor{color_racinggreen}{HTML}{1B9569} %racing green
%-- TU colors
\definecolor{color_TU_blue}{HTML}{006699}
\definecolor{color_TU_lightblue}{HTML}{7FB2CC} 
\definecolor{color_TU_green}{HTML}{379237} 

